Asymptotic normality and optimality in nonsmooth stochastic approximation

In their seminal work, Polyak and Juditsky showed that stochastic approximation algorithms for solving smooth equations enjoy a central limit theorem. Moreover, it has since been argued that the asymptotic covariance of the method is best possible among any estimation procedure in a local minimax sense of H\'{a}jek and Le Cam. A long-standing open question in this line of work is whether similar guarantees hold for important non-smooth problems, such as stochastic nonlinear programming or stochastic variational inequalities. In this work, we show that this is indeed the case.

==> annals_stat - V1/liweimacros.tex <==
\numberwithin{equation}{section}
%%%%%%%%%% Math %%%%%%%%%%%%%%%
\newcommand{\const}{a}

\newcommand{\localmu}{\mu}
\newcommand{\E}{{\bf E}}
\newcommand{\R}{{\bf R}}
\DeclareMathOperator*{\LS}{Limsup}
\newcommand{\lipschitz}{\mathrm{Lip}}
\newcommand{\localconstant}{C}
\newcommand{\perturbbound}{\mathsf{}}
\newcommand{\gbound}{\mathsf{L}}
\newcommand{\projshort}{P}
\newcommand{\error}{E}
\newcommand{\verdier}{Verdier~}
%\newcommand{\projshort}{\proj}
\newcommand{\interior}{\mathrm{int}\; }
\newcommand{\xkball}{\ball{p}{\delta_p}}
\newcommand{\ykball}{\ball{p}{\epsilon_p/2}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\ip}[1] {\langle #1 \rangle }
\newcommand{\norm}[1] {\left \| #1 \right \|}
\newcommand{\inclu}[0] {\ar@{^{(}->}}
\newcommand{\conn}{{\scriptstyle \#}}
\newcommand{\Aut}[1] {\text{Aut}_{#1}}
\newcommand{\Rank}{\text{Rank }}
\newcommand{\Ker}{\text{Ker }}
%\newcommand{\vec}{\text{Vec }}
\newcommand{\Dim}{\text{dim }}
\newcommand{\spann}{\text{span}}
\newcommand{\im}{\text{Im }}
\newcommand{\gph}{{\rm gph}\,}
\newcommand{\diag}{{\rm diag}}
\newcommand{\dist}{{\rm dist}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\trace}{\mathrm{Tr}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\lip}{\mathrm{lip}}
\newcommand{\var}{\mathrm{var}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\pfail}{p_{\mathrm{fail}}}
\newcommand{\st}{\text{subject to:}}
\newcommand{\minimize}{\mathrm{minimize}}
\newcommand{\maximize}{\mathrm{maximize}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\SOC}{\mathrm{SOC}}
\newcommand{\sym}{\mathbb{S}}
\newcommand{\epi}{\mathrm{epi}\,}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\range}{\mathrm{range}}
\newcommand{\cl}{\mathrm{cl}\,}
\newcommand{\bdry}{\mathrm{bdry}\,}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\val}{{\rm \texttt{val}}}
\newcommand{\aval}{{\rm \texttt{a-val}}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\modelell}{l}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\mE}{\mathbf{E}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\I}[1]{\mathbb{I}_{\left\{#1\right\}}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\nnorm}[1]{\| #1 \|_*}
\newcommand{\fnorm}[1]{\| #1 \|_{F}}
\newcommand{\ceil}[1]{\left \lceil #1 \right \rceil }
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor }
\newcommand{\1}{\mathbf{1}}
%%%%%%%%% Convex Analysis %%%%%%%%%
\newcommand{\prox}{\mathrm{prox}}
\newcommand{\proj}{P}
\newcommand{\dom}{\mathrm{dom}\,}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\ls}{\operatornamewithlimits{limsup}}
\newcommand{\Diag}{{\rm Diag}}
\newcommand{\argmax}{\text{argmax}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\polylog}{\text{polylog}}
%%%% Probability %%%%%%%%%%%%%%%%%
\newcommand{\Prob}{\text{\textbf{Pr}}}
\newcommand{\Expect}{\mathbb{E}}
\newcommand{\matrx}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\opnorm}[1]{\left\|#1\right\|_{op}}
\newcommand{\expect}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\prob}[1]{\mathbb{P}\left(#1\right)}
\newcommand{\dotp}[1]{\left\langle #1\right\rangle}
\newcommand{\mw}{\mathbf{w}}
\newcommand{\mz}{\mathbf{z}}
\newcommand{\mb}{\mathbf{b}}
%%%%%%%% Theorems %%%%%%%%%%%%%
\newtheorem{thm}{Theorem}[section]
\newtheorem{exercise}{thm}[section]
\newtheorem{definition}[thm]{Definition}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{pa}{Part}
\newtheorem{subclaim}{Subclaim}
\newtheorem{assumption}{Assumption}
\renewcommand*{\theassumption}{\Alph{assumption}}
%%%%%%%%%%Paper%%%%%%%%%%%%%%%
\newcommand{\ma}{\mathbf{a}}
\newcommand{\mx}{\mathbf{x}}
\newcommand{\me}{\mathbf{e}}
\newcommand{\mX}{\mathbf{X}}
\newcommand{\mM}{\mathbf{M}}
\newcommand{\mmu}{\mathbf{u}}
\newcommand{\mv}{\mathbf{v}}
\newcommand{\rub}{\gamma_{\text{ub}}}
\newcommand{\gt}{\nabla \rho(\mx)}
\newcommand{\Lip}{\mathsf{L}}
\newcommand{\lb}{\texttt{lb}}
\newcommand{\ub}{\texttt{ub}}
\newcommand{\thr}{\texttt{thr}}
\newcommand{\gr}{\texttt{gr}}
\newcommand{\cushion}{\hat \gamma_\ub}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\stab}{\texttt{stab}}
\newcommand{\last}{\texttt{last}}
\newtheorem{remark}{Remark}
\newtheorem{notation}{Notation}
\newtheorem{example}{Example}[section]
\renewcommand*{\thepa}{\alph{pa}}
\newcommand{\brac}[1]{\left[ #1 \right]}
\newcommand{\paren}[1]{ \left( #1 \right) }
\theoremstyle{remark}
\newtheorem{claim}{Claim}

%%%%%%%%%%%%%%Saddle paper%%%%%%%%%%%%%%%%
\newcommand{\sphere}{\mathbb{S}}
\newcommand{\unif}{\text{Unif}}
\newcommand{\discrete}{k}
\newcommand{\continuous}{t}
\newcommand{\perturb}{\nu}
\newcommand{\stepsize}{\alpha}
\newcommand{\subgrad}{v}
\newcommand{\nonsmsg}{w}
\usepackage{mathtools}
\usepackage[boxruled]{algorithm2e}

